Ising-Based Louvain Method: Clustering Large Graphs with Specialized Hardware

Recent advances in specialized hardware for solving optimization problems such quantum computers, quantum annealers, and CMOS annealers give rise to new ways for solving real-word complex problems. However, given current and near-term hardware limitations, the number of variables required to express a large real-world problem easily exceeds the hardware capabilities, thus hybrid methods are usually developed in order to utilize the hardware. In this work, we advocate for the development of hybrid methods that are built on top of the frameworks of existing state-of-art heuristics, thereby improving these methods. We demonstrate this by building on the so called Louvain method, which is one of the most popular algorithms for the Community detection problem and develop and Ising-based Louvain method. The proposed method outperforms two state-of-the-art community detection algorithms in clustering several small to large-scale graphs. The results show promise in adapting the same optimization approach to other unsupervised learning heuristics to improve their performance.

==> sections/Infrastructure.tex <==
% Cut from methods.tex



% \subsection{Infrastructure}
% \subsubsection{Software}
% The entire clustering package and the experiments were developed in Python 3.7 \cite{van2007python}: graphs were modeled with NetworkX v2.4 \cite{hagberg2008exploring} and python-iGraph v0.8.2 \cite{csardi2006igraph}, arrays were handled with NumPy v1.18 \cite{van2011numpy} and SciPy v1.4.1 \cite{virtanen2020scipy}, QUBOs were solved using Fujitsu's Digital Annealer Firmware \cite{aramon2019physics}, and LeidenAlg v0.8.1 \cite{traag2019louvain} was used for running the Leiden algorithm. Thomas Aynaud's python-louvain module \cite{aynaud-python} was used both as the basis for developing the Ising-Louvain algorithm and for running the original Louvain algorithm.
% \subsubsection{Hardware}
% The experiments were run on an Intel Xeon E5-2699 v3 (2.30 GHz) CPU with 125 GiB of available system memory, and Fujitsu's Digital Annealer v3.4 was used as the hardware to solve the QUBOs. Fujitsu's Digital Annealer v3.4

==> sections/da1sec.tex <==
 \begin{table}[t]
    \centering
    \caption{Summary of the results of running Louvain, Leiden, and Ising-Louvain on the benchmark graphs, along with statistics of the solver} % \added[id=hm]{do we have DA results?}}
\label{tab:1}
    \begin{tabular}{lcccccc|cc}%cc}
        \multicolumn{1}{l}{} & \multicolumn{6}{c}{\textbf{Optimal Modularity Results}} & \multicolumn{2}{c}{\textbf{Solver Stats}}\\
     \textbf{Graph} & \textbf{Leiden} & \textbf{\#Clusters} & \textbf{Louvain} & \textbf{\#Clusters} & \textbf{Ising-Louvain} & \textbf{\#Clusters} & \textbf{Avg QUBO Size} & \textbf{\#Solver-Calls}\\% & \textbf{Runtime(s)} & \textbf{Runtime/Call}\\
    \hline
    
    KarateClub & 0.4198 & 4 & \textbf{0.4198} & 4 &\textbf{ 0.4198 }& 4 & 75 & 4 \\%& 15.2 & 3.8\\
    Meredith & 0.7457 & 8 & \textbf{0.7571} & 10 & \textbf{0.7571} & 10 & 164  & 4 \\%& 15.6  & 3.9\\
    LesMiserables & 0.5600 & 6 & \textbf{0.5667 }& 6 &\textbf{ 0.5667 }& 6 & 85 & 14 \\%& 102.2 & 7.3\\
    Facebook & 0.8356 & 16 & 0.8350 & 16 & \textbf{0.8358 }& 17 & 19 & 584 \\%& 2570 & 4.4\\
    Autonomous & \textbf{0.6662} & 36 & 0.6553 & 37 &0.6572& 35 & 7 & 1626 \\%& 18536 & 11.4\\
    LastFM &\textbf{0.8170} & 27 & 0.8155 & 29 & 0.8168& 29 & 16 & 19036\\% & 218914 & 11.5\\
    arXiv & \textbf{0.7759 }& 476 & 0.7699 & 479 & 0.7756 & 473 & 11 & 36373\\% & 24090 & 6.0\\
    arXiv2 & 0.6649 & 315 & 0.6622 & 317 & \textbf{0.6650 }& 324 & 32 & 115898\\%& 7552 & 0.1\\
    AstroPh & 0.6367 & 324 & 0.6309 & 324 & \textbf{0.6378 }& 328 & 44 & 351410\\% & 38282 & 0.1\\
    Enron & 0.6265 & 1242 & 0.6204 & 1241 & \textbf{0.6285 }& 1272 & 23 & 146451\\% & 35504 & 0.2\\
    DBLP & \textbf{0.8301} & 221 & 0.8220 &    197    & 0.8231 & 252 & 13 & 204893\\% & 1158612 & 0.1\\
    Amazon & \textbf{0.9309}  & 391 & 0.9263 & 246 &0.9277& 299 & 14 & 7812919\\% & 1048961 & 0.1\\
    \end{tabular}%
%}%
 \end{table}
